High-Resolution Be Aware! Improving the Self-Supervised Real-World Super-Resolution

Self-supervised learning is crucial for super-resolution because ground-truth images are usually unavailable for real-world settings. Existing methods derive self-supervision from low-resolution images by creating pseudo-pairs or by enforcing a low-resolution reconstruction objective. These methods struggle with insufficient modeling of real-world degradations and the lack of knowledge about high-resolution imagery, resulting in unnatural super-resolved results. This paper strengthens awareness of the high-resolution image to improve the self-supervised real-world super-resolution. We propose a controller to adjust the degradation modeling based on the quality of super-resolution results. We also introduce a novel feature-alignment regularizer that directly constrains the distribution of super-resolved images. Our method finetunes the off-the-shelf SR models for a target real-world domain. Experiments show that it produces natural super-resolved images with state-of-the-art perceptual performance.

==> figures/lway_lim.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.95\linewidth]{figures/lway_limi.pdf}
    % \InsertSubfigWithCap{0.50}{figures/lway_limi_a.pdf}{cap}
    % \InsertSubfigWithCap{0.40}{figures/lway_limi_b.pdf}{cap}
    \caption{Two drawbacks of simple LR reconstruction. LR images are interpolated for better visuals. In the left example, when $e_d$ cannot reproduce degradation in LR input $X$, the ground-truth $Y_{gt}$ yields worse reconstruction performance (PSNR/LPIPS) compared to the $f_X(Y_{gt})$, where $f_X$ is the same type of degradation in $X$. \YZ{combine to fig 3}.
    % ~\AY{what scale factor are we actually working with?  is the image shown realistic and correct?  the "x reproduce" is confusing}
    }
    \label{fig:lway_lim}
\end{figure}

==> sec/1_intro_old.tex <==
\section{Introduction}
~\AY{i'd be happy if we can reduce some of the acronyms in our text.  there are too many and they all look very similar, so it becomes hard to distinguish (LR, HR, SR).  especially challenging is the LR vs. LRN; then there is also LWay, and the GT... it's ugly to read.  pick a few (perhaps LR and HR) and write out the rest?}

\label{sec:intro}
Image super-resolution reconstructs high-resolution (HR) images from low-resolution (LR) ones. Real-world LR data contains various other degradations, \eg blur, noise, and compression, with unknown formulations. Due to the cost and difficulty of collecting paired data in real-world cases, supervised methods for real-world super-resolution still rely primarily on synthetic data. However, synthetic data have some domain gaps from real-world data, and they cannot be used naively without ~\AY{XX}.  ~\AY{YY}
As such, self-supervised SR methods using \hl{only} LR images are crucial for directly learning from real-world domains.

\input{figures/teaser}
Designing effective self-supervision losses is extremely challenging for super-resolution. Previous methods mainly construct pseudo data pairs from the LR inputs~\cite{shocher2018zero,gu2019blind,soh2020meta,deng2023efficient, cheng2020zero}. Those methods degrade the original low-resolution image to a even lower resolution pseudo-LR input and use the original image as the super-resolved target. The degradations for producing the pseudo-LR inputs determine the effectiveness. Great efforts have been made to reproduce the degradation kernels in the original low-resolution inputs~\cite{gu2019blind,deng2023efficient,cheng2020zero}. However, the reproduced kernels %from those methods are 
derived from predefined functions, \eg Gaussian blurring and Gaussian noise, which do are often insufficient to capture the true extent of real-world degradations. %cannot express real-world ones well and distract the SR model from solving the original degradation.


% The recent DegAE [18] proposes a pretraining paradigm for image enhancement tasks, which learns degradation embeddings through an Autoencoder.

In place of explicitly defined degradation kernels, the recent DegAE~\cite{liu2023degae} proposed to implicitly represent image degradations through a {degradation embedding}.  The embeddings are learned in the form of an autoencoder through self-reconstruction on the degraded input. %The auto-encoder of~\cite{liu2023degae} 
This was then extended by LWay~\cite{chen2024low} 
% a low-resolution reconstruction network (LRN) 
for self-supervised super-resolution.
LWay first uses synthetic paired data to pretrain a degradation encoder and a downsampling decoder (see Fig.~\AY{X}).  The encoder projects the LR input into a degradation embedding.  The decoder downsamples and degrades an HR image into a LR image, conditioned on the degradation embedding. These structures are then frozen, and used to support the fine-tuning of an off-the-shelf SR model targeting a real-world domain. For both the pre-training and the fine-tuning, LWay uses a reconstruction loss between the low-resolution input and the reconstructed low-resolution output from the decoder.

%inspiredly adapts the Autoencoder to the LR reconstruction network (LRN) for self-supervised SR. 
% before using it to 
% for reconstructing LR inputs based on its degradation embedding and corresponding ground-truth (GT) images. 
% degrades \hl{the ground-truth HR} images to LR ones based on the degradation embeddings of the LR s. 
% The pretrained LRN is frozen and used for 
% support the 
%\hl{requiring the super-resolved images and degradation embedding to reconstruct LR inputs} 
% \YZ{one sentence for why this is a paradigm worth to follow}
% \st{The LR reconstruction leverages informative degradation embeddings, relieving self-supervised SR from ineffective kernel estimations.}

~\AY{I think we need an explicit statement (here? you choose) mentioning (1) why LWay is still good, especially for the real-world setting and (2) we build upon their framework.  also, i think we might want to meniton somehwere int he previous two paragraphs and or here again, explicitly that we are targeting hte real-world superresolution problem.  the previous paragraphs are rather generic and don't really say what problem we are addressing.}

However, simply reconstructing the low-resolution image %as done by LWay~\cite{chen2024low} 
has two specific drawbacks making it insufficient for super-resolution. 
First is the assumption that the degradation embedding can fully encode the degradation specifics of LR inputs. {Furthermore, it is assumed that reconstructing the low-resolution input during fine-tuning will lead to high-fidelity super-resolved images on par with the ground-truth HR used in pre-training.}  Yet in real-world settings, the degradation embeddings are not always sufficient to reproduce the input degradations. The implications then arise during fine-tuning, where the degradation encoder and downsampling decoders are frozen. The only way to compensate for a non-ideal degradation embedding is for the super-resolution model to reconstruct a non-ideal and likely degraded high-resolution image. ~\AY{can we call this a form of collapse? give name.}
% In such cases, \hl{HR images need to contribute} to degradation reproduction \ie, finetuning the SR model for good LR reconstructions \hl{can degrade the HR images to reproduce LR degradations.}
\input{figures/lway_lim}
Such a phenomenon is highlighted in the contradiction shown in~\cref{fig:lway_lim}, where passing a ground truth HR through the decoder leads to lower reconstruction performance than a blurry HR image.

% shows an example where using a ground truth image with the same type of blur as the low-resolution input yields that the GT image with the same type of blur as the LR yields higher LR-reconstruction performance than the original GT image.

% {Secondly, LR reconstruction is ineffective in enhancing high-frequency information for HR images due to the ill-posedness of SR.
% As in \cref{fig:lway_lim}, ill-posedness refers to multiple HR images corresponding to a single LR image due to downsampling~\cite{wang2020deep,jo2021tackling}. 

A second drawback is that LR reconstruction alone is insufficient to guide the learning towards high-quality HR outputs.  ~\AY{make argument for why we need XX for high-quality outputs, this is typically incorporated through XYZ in other SR methods.} 
inherent in the LR reconstruction scheme -- 
\hl{The effectiveness of LR reconstruction is limited for lost high-frequency information, which is essential for being natural.}~\AY{expand on this point: existing setup only cares about LR, so has limited effect on the HR.  but human eye relies on high frequency to look good. this is incorporated into almost all SR methods in various ways through X Y Z, but current method doesn't have.}
% In practice, the sharpness of super-resolved images always drops after applying LWay.

To tackle these two drawbacks, this paper strengthens awareness of high-resolution images.  It uses ~\AY{unpaired HR images} to improve the LR reconstruction objective from two perspectives. 
First, to prevent ~\AY{HR collapse} during fine-tuning, we want to make the \hl{LRN} aware of the super-resolution quality.
Specifically, we adjust the degradation embedding through \hl{a controller $s$}. The controller is defined by a new High-resolution Quality Indicator (HQI) to indicate the quality of super-resolved images.
For low-quality SR images, we raise the extent of degradation to enlarge the contribution of degradation embedding in reproducing LR degradations, so that pursuing LR reconstruction is \hl{deactivated} from degrading SR images.

Second, to tackle ~\AY{the drawback due to ill-posedness}, we propose a novel Feature-Alignment Regularizer (FAR) for the %directly applied to 
HR images. Previously, model-based SR methods~\cite{yang2008image,timofte2015a+,liu2013bayesian} %has leveraged LR reconstruction objective but with an extra 
applied a prior $\Phi(y)$ on the super-resolved image $y$, such as sparsity~\AY{, or X}. % to %, regularizing 
%encourage the characteristics of $y$ to be natural. 
Inspired by these methods, we design FAR to encourage the super-resolved images to have characteristics that resemble natural images. %have natural characteristics. Traditional methods design $\Phi(y)$ to constrain simple features such as sparsity. Instead, FAR leverages a self-supervision loss on HR images to capture distribution features.  
It has been studied that \hl{an optimized} self-supervised \hl{loss can detect} the distribution shift between the training data and the testing data~\cite{tsai2023convolutional}. Therefore, during pretraining, we also encode the HR image and align the image features to that from another pretrained encoder, \eg CLIP image encoder~\cite{radford2021learning}. 
When finetuning the SR model, the same alignment relationship is optimized for the super-resolved images. As such, FAR closes the disparity between the distribution of the SR outputs and the HR images for LRN pretraining, which are ground truths with a natural image distribution.


Through the two novel designs, our method equips the LR reconstruction objective with awareness of HR quality. In summary, the contributions of this paper are three-fold:
\begin{itemize}
    \item {We adjust the degradation extent by the SR quality, relieving the LR reconstruction from degrading HR images for reconstruction performance.}
    \item {To complement the defects due to ill-posedness, we propose a novel Feature-Alignment Regularizer to constrain HR image for natural distribution.}
    \item Experiments on multiple datasets show that our method improves off-the-shelf SR models perceptually and objectively and achieves state-of-the-art performances for essential perceptual quality.
\end{itemize}



~\AY{suggestion for new storyline: we want to rw-sr thru self-supervision (+motivation why self-supervision).  Existing methods for self-supervision focus on LR-reconstruction, but this is problematic because LR-reconstruction inherently will ignore information about HR which is crucial for good quality.  existin gmethods for self-supervision also like to synthesize or learn kernels explicitly; results are not good, maybe better to use embeddings (borrow some motivationf rom degAE/Lway, why embeddings are good.)  using embeddings naively, within the self-supervised manner might lead to collapse, we can fix.

}

==> sec/3_method.tex <==

\section{Super-Resolution Revisit}
\label{sec:revist}

\subsection{Standard v.s. Real-World Super-Resolution}
Consider a super-resolution model $\mathrm{M}$ which restores an HR image $\hat{Y}\in\Size{aH}{aW}{N}$ from the LR input $X\in\Size{H}{W}{N}$, where $a$ is the scaling factor and $N$ is the number of color channels. In most SR schemes, paired training data is synthesized by downsampling a ground-truth image $Y^s_{gt}$:
\begin{equation}
X^s = f_{\downarrow}(Y^s_{gt}),
\end{equation}
\noindent to the LR counterpart $X^s$. For standard SR, $f_{\downarrow}$ is a simple and fixed operation such as bicubic downsampling. For real-world SR, $f_{\downarrow}$ is more complex and incorporates degradations other than downsampling. 
{The real-world degradations are complex without known formulations, while degradations in data from the same source (\eg a specific camera, or an Internet source) are consistent.}
~\AY{explain how degradations unknown, complex, and many will approximate what is encountered in real-world}

It is very challenging to collect paired real-world datasets. Existing datasets only include data from a few camera sources and the HR images also suffer from blur. 
~\AY{existing datasets are XX - mention how dataset x, gt is fuzzy.} Therefore, in most real-world SR set-ups, the LR images $X^r$ are available \hl{and the corresponding HR ground truth $Y^r_{gt}$ are assumed absent.} As such, supervised learning for a real-world domain is infeasible.
% Therefore, the real-world SR methods always assume that the paired ground truth for $X^r$ is unavailable and supervised learning on the real-world domain is infeasible.

Many SR methods synthesize paired data with complex and random degradations, \eg using the second-order degradation pipeline~\cite{wang2021real}. Trained on such data, SR models blindly generalize to diverse input conditions. However, specific adaptation for the encountered real-world data always benefits compared to a ``jack-of-all-trades'' model~\cite{zhang2023crafting,zhang2024real}.
In this paper, we finetune the generalized SR models for better performance on real-world data.  
~\AY{rethink our strategy of talking about how real-world methods rely on synthetic and real-world data, hence the notation for $X^s$ and $X^r$}
% \hl{Most self-supervised SR methods} \hl{directly reproduce degradation kernels of LR images}. 

\subsection{Self-Supervised Super-Resolution}
~\AY{I recommend introducing the following differently - separate the concept of autoencoder (which is mostly architectural and supports the aim of self-supervision) vs. the latent mapping of the real-world degradations.  This current paragraph's focus should be on the latent modelling of the degradation itself. previous methods model degradation explicitly as kernels.  the new paradigm is to model the image content and degradation separately. the degradation is encoded as an embedding vector.  the aim of self-supervision networks is to reconstruct the LR image}
% Most unsupervised SR methods~\cite{wei2021unsupervised,zhang2024pairwise} use the $X^r$ from a target real-world domain and a set of unpaired high-resolution data $Y_{gt}^s$, while 
\tc{Self-supervised methods~\cite{cheng2020zero,shocher2018zero} usually only use real-world LR $X^r$ and optimize the SR model for a specific test image or a real-world domain consisting of LRs with consistent real-world degradation. 
The recent method uses external HR images but only in the pretraining stage~\cite{chen2024low}, not in performing optimization on real-world data. 
% Similarly, we synthesize paired data from $Y_{gt}^s$ through second-order degradation for pretraining. When fine-tuning the SR model, only real-world low-resolution images are required.
% Existing self-supervised SR methods approximate the degradation in $X^r$ by predefined kernels and then construct training pairs from $X^r$. 

DegAE~\cite{liu2023degae} proposed a pretraining paradigm for image enhancement tasks to encode image degradations into a high-dimensional embedding; this approach is adapted by LWay~\cite{chen2024low} for self-supervised super-resolution with an LR reconstruction network (LRN). 
The LRN consists of a degradation encoder $E_{deg}$, an image encoder $E_{img}$, and a decoder $D$. The decoder reconstructs the LR input $\hat{X}$ based on the degradation embedding $e_d$ and image content feature $e_{im}$ ~\AY{XX}:
% \begin{equation}
%     \hat{X} = D(e_d, E_{img}(Y_{gt})), \quad\text{where } e_d = E_{deg}(X).
% \end{equation}
\begin{equation}
\begin{aligned}
    \hat{X} &= D(e_d, e_{im}),\quad\text{and } \\e_d &= E_{deg}(X), e_{im}=E_{img}(Y),
\end{aligned}
\end{equation}
where $e_d\in\mathbb{R}^{C_d}$, $e_{im}\in\mathbb{R}^{C_i\times\!H_i\times\!W_i}$, and $E_{img}$ is set as a identify mapping in LWay.

LRN is first pretrained on external paired data $\{X^s, Y^s_{gt}\}$ for the LR reconstruction objective~\AY{explicitly mention here, pertaining is to learn which parts}:
\begin{equation}
\begin{aligned}
    \theta^*_{pt} &= \arg\min_{\theta_{pt}} \mathcal{L}_{rec}(D(e_d, e_{im}), X^s),\quad\text{and } \\&e_d = E_{deg}(X^s), e_{im}=E_{img}(Y_{gt}^s),
    \label{eq:rec_pt}
\end{aligned}
\end{equation}
where $\theta_{pt}$ is the parameters of full LRN. 

The finetuning stage generalizes an off-the-shelf SR model $\mathrm{M}$ to a \hl{real-world domain} through reconstructing the LR sample $X^r$:
\begin{equation}
\begin{aligned}
    \theta^*_{ft} &= \arg\min_{\theta_{ft}} \mathcal{L}_{rec}(D(e_d, e_{im}), X^r),\quad\text{and } \\&e_d = E_{deg}(X^r), e_{im}=E_{img}(\mathrm{M}(X^r)),
\end{aligned}
\label{eq:rec}
\end{equation}
where LRN is frozen and $\theta^*_{ft}$ is optimized parameters from the SR model $\mathrm{M}$.

The LR reconstruction objective \cref{eq:rec} trusts $e_d$ in reproducing degradations in $X^r$ and therefore targets $\mathrm{M}(X^r)$ at as high-quality as HR images in the pretraining stage. However, \cref{eq:rec} does not align with the aim of super-resolution well without direct awareness of high-resolution.}

\section{Methodology}

\begin{figure*}[h!]
    \begin{subfigure}[t]{0.43\linewidth}
        \includegraphics[width=\textwidth]{figures/overview_pt.pdf}
        \subcaption{Pretraining of LR reconstruction network on synthetic data. }
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.47\linewidth}
        \includegraphics[width=\textwidth]{figures/overview_ft.pdf}
        \subcaption{Finetuning of SR model $\mathrm{M}$ on real-world data.}
    \end{subfigure}
    \caption{Overview of how our method strengthens the awareness of HR images in the self-supervision. In each stage, only colored models or modules are optimized. (a) The pretraining of LRN. The degradation encoder $E_{deg}$, image encoder $E_{img}$, decoder $D$ and parameters in $FAR$ are optimized with $\mathcal{L}_{rec}$ and $\mathcal{L}_{far}$. Controller $s$ rescales $e_d$. LR input $X^s$ (interpolated for better visuals) is synthesized from natural high-resolution image $Y^s_{gt}$. (b) Finetuning of super-resolution model $\mathrm{M}$. Given a real-world LR image, $X^r$, we input the HR image $\mathrm{M}(X^r)$ to $E_{img}$ and $E_{clip}$. Only parameters in $\mathrm{M}$ are finetuned by $L_{rec}$ and $\mathcal{L}_{far}$. The relationships between $s$ and HQI are different in finetuning from pretraining. 
    ~\AY{minor, but can we use a non-chinese text example? make the pre-training and fine-tuning headers bigger and state explicitly, on synthetic vs. real-world data; alternatively, separate them into subplots (a) and (b); for legend, linear *layer; what is the meaning of the green parts?  I assume it is the learning part?  if so why is the $e_d$ vector itself coloured? if so, is the orange portion also trained? (coloured for learning, grey for frozen?)}}
    \label{fig:overview}
\end{figure*}
\label{sec:methodology}

\tc{\cref{fig:overview} is an overview of our method. The key novelty is incorporating HR images in the self-supervision for finetuning \YZ{for xxx and xxx}.}
The pretraining stage on the left optimizes the LR reconstruction network with the novel controller $s$ and a feature-alignment regularizer (FAR). The finetuning stage on the right adapts an off-the-self SR model for the test domain with the LR reconstruction loss and FAR. {We begin by general description of using HR in the self-supervision loss in \cref{subsec:overview}.} The methodology is completed by {how we define $s$ and detail designs of FAR}in \cref{subsec:HQI} and \ref{subsec:FAR}. % completes the methodologyfurther explains the details of novel designs.

\subsection{Overview}
\label{subsec:overview}
% \YZ{Motivation}
~\AY{one paragraph outlining the drawback of the straight-forward approach. collapse, etc. we discussed during last mtg. to give motivation for why we need to have some prior on the HR image.  can also highlight the need for the $s$ vector for controlling hte extent of degradation, etc.}

{The LR reconstruction in \cref{eq:rec} is straightforward by focusing LR images only in the self-supervision loss. Nevertheless, a good reconstruction of LR inputs correlates loosely with good-quality high-resolution images. There are two specific drawbacks. First, when the degradation embedding $e_d$ fails to reproduce degradations in $\hat{X}$, a good LR reconstruction indicates the HR image, on the other hand, contributes to the degradation reproduction. Second, even with ideal degradation embedding, high LR reconstruction performance does not ensure a natural HR image due to the ill-posedness of the SR problem.}

To tackle the above limitations, we strengthen the awareness of HR images in the self-supervision loss. 
{Our first motivation is to alleviate the HR image from contributing to the reproduction of degradations.}\YZ{further explain the specific collapse for LR reconstruction scheme} 
To achieve this aim, we design a High-resolution Quality Indicator (HQI) to monitor the quality of HR image $M(X^r)$. For low-quality $M(X^r)$, we expect the $e_d$ to contribute more to relieve the LR reconstruction objective from the risk of degrading $M(X^r)$. Therefore, we generate $s$ based on HQI to control degradation extent, the primary attribution of degradations, and raise the degradation extent for low-quality $M(X^r)$. 

{Second, we introduce a Feature-Alignment Regularizer (FAR) inspired by the prior in model-based SR methods~\cite{liu2013bayesian,yang2008image,timofte2015a+}.
FAR directly regularizes the feature of HR images to have characteristics of natural images. Regularizers in model-based SR only constrain simple characteristics related to natural image, \eg sparsity and total variance~\cite{timofte2015a+,ulyanov2018deep}.
A recent paper observed that self-supervision loss optimized for a specific data distribution will increase when data distribution shifts~\cite{tsai2023convolutional}.
Similarly, we design FAR leveraging self-supervision on HR images. 
FAR calculates the statistical similarity between features encoded by $E_{img}$ and another pretrained image encoder $E_{clip}$, \eg CLIP image encoder. 
The pretraining stage optimizes such similarity for natural images, \ie ground truth $Y^s_{gt}$.
The finetuning stage enforces the same alignment relationship for super-resolved image $\mathrm{M}(X^r)$ to narrow the disparity between characteristics of $\mathrm{M}(X^r)$ and natural images.

As a summary, the finetuning stage of our method optimizes parameters of $\mathrm{M}$ with the help of controller $s$ and regularizer $\Phi$ involved:
\begin{equation}
\begin{aligned}
\theta^*_{ft} =& \arg\min_{\theta_{ft}} \mathcal{L}_{rec}(D(s\cdot e_d, e_{im}), X^r) \\ &+ \lambda_r\Phi_{far}(M(X^r)),
\quad\text{and } \\&e_d = E_{deg}(X^r), e_{im}=E_{img}(\mathrm{M}(X^r)),
    % E\|D(s\cdot e_d,\:E_{img}(\mathrm{M}(X^r)))-X^r\| \\+ \lambda_r\Phi(E_{img}(\mathrm{M}(X^r))),
    \label{eq:overview}
\end{aligned}
\end{equation}
where $s$ controls the degradation extent and $\Phi(\cdot)$ refers to FAR.
Following LWay~\cite{chen2024low}, $\mathcal{L}_{rec}$ is implemented as $\ell_1$ loss and LPIPS loss. 
% in the finetuning stage, $\mathcal{}$ is applied to the high-frequency (HF) part of $X$ and $X^r$. 
Detailed definitions of $\mathcal{L}_{rec}$ are shown in Supplementary \cref{subsec:supp_loss}.

The pretraining stage also includes $s$ and FAR.
\cref{subsec:HQI} and \cref{subsec:FAR} explain the details of controller $s$ and FAR in the pretraining and finetuning stages.}

\subsection{Controller $s$}
\label{subsec:HQI}
As introduced in \cref{subsec:overview}, the aim of controller $s$ is to adjust the degradation extent based on the quality of super-resolved images. 
{However, the quality of $\mathrm{M}(X^r)$ cannot be measured directly without available ground-truth $Y_{gt}^r$. Considering the motivation of engaging SR quality, \ie alleviating the HR image from contributing to the reproduction of degradation, we use the similarity between $X^r$ and $\mathrm{M}(X^r)$ as the indicator. When $M(X^r)$ has \hl{a higher similarity to LR input}, it indicates the more degradations in $\mathrm{M}(X^r)$.} In practice, HQI is defined as:
\begin{equation}
\begin{aligned}
    \text{HQI}(X^r,\hat{Y}^r) &= 1 - \text{LPIPS}(f_\uparrow(X^r), \hat{Y}^r), \\
    \hat{Y}^r &= \mathrm{M}(X^r)
\end{aligned}
\end{equation}
where $f_\uparrow$ is bicubic upsampling to align spatial resolution of $X^r$ to $\mathrm{M}(X^r)$, and LPIPS~\cite{zhang2018unreasonable} calculates the cosince \textit{distance} $d\in [0,1]$ between image features.

{In the finetuning stage, when $X^r$ and $\mathrm{M}(X^r)$ are close, \ie \textit{high} HQI, we raise the degradation extent to lower the need for degrading HR images to reconstruct LRs.
The pretraining stage also uses controller $s$ to avoid the gap between the training and using of LRN. 
As $Y^s_{gt}$ in the pretraining stage is ground-truth, the similarity between $X^s$ and $Y^s_{gt}$ reflects the "ground-truth'' degradation extent, \ie high similarity should correlate to low degradation extent. 
The controller $s$ in \cref{eq:overview} is thus defined differently for the pretraining and finetuning stages:
\begin{equation}
 s =\begin{cases}
    \mathbf{n} + (1-\text{HQI}(X^s, Y^s_{gt})),  & \text{pretraining}\\
    \mathbf{n} + \text{HQI}(X^r, \hat{Y}^r),   & \text{finetuning}
\end{cases}.
\label{eq:s}
\end{equation}
The vector $\mathbf{n}$ is a $C_d$-dimensional random vector and $\mathbf{n} \sim \mathcal{N}(\mathbf{0}, \mathbf{I})$, which helps the robustness.}

\subsection{Feature-Alignment Regularizer (FAR) }
\label{subsec:FAR}
\begin{figure}
    \centering
    \includegraphics[width=0.85\linewidth]{figures/far.pdf}
    \caption{Details of the Feature-Alignment Regularizer. }
    \label{fig:far}
\end{figure}
% Feature-alignment-based regularizer (FAR) 
\tc{To supplement the LR reconstruction objective, we design FAR to constrain the disparity between the characteristics of super-resolved images and natural images.}
It applies \hl{a self-supervision loss} to HR images which pursues the alignment between features of the same HR image $Y$ encoded by $E_{img}$ in \cref{eq:overview} and a pretrained image encoder $E_{clip}$ from CLIP~\cite{radford2021learning} model:
\begin{equation}
\begin{aligned}
    \Phi_{far}(Y) = \mathcal{L}_{far}(e_{im}, e_{cl}), \quad\text{and}\\ e_{im}=E_{img}(Y),\: e_{cl} = E_{clip}(Y), 
\end{aligned}
\label{eq:im_feat}
\end{equation}
where $e_{im}\in\Size{C_i}{H_i}{W_i}$ and $e_{im}\in\Size{C_c}{H_c}{W_c}$.

The calculation of $\mathcal{L}_{far}$ should focus on statistical differences between feature maps so that its value changes can effectively reflect distribution shifts.
As in \cref{fig:far}, 
% the decoder takes degradation embedding $e_d$ and image embedding extracted by $E_{img}$ as inputs. FAR is designed as a regularizer on the \hl{statistical descriptors of the image embedding $e$}:
we design a statistical descriptor based on the Gram Matrix~\cite{gatys2016image} of image feature $e\in\Size{C}{H}{W}$: 
\begin{equation}
\begin{aligned}
    &S_{avg}(e) = \text{AvgPool}(G(e)), \\&S_{max}(e) = \text{MaxPool}(G(e)),
\end{aligned}
\label{eq:stat_des}
\end{equation}
where $G$ calculates the Gram Matrix, \ie channel correlation of feature maps, and  $G(e)\in\mathbb{R}^{C\times\!C}$. The Gram matrix of a deep feature focuses on the statistical features rather than image content~\cite{gatys2016image}.
We use the average and maximum values of each channel's correlation to others as the statistical descriptor, and both $S_{avg}$ and $S_{max}$ are of size $\mathbb{R}^C$. 

We then define $\mathcal{L}_{far}$ as difference between statistical descriptors calculated for $e_{im}$ and $e_{cl}$ in \cref{eq:im_feat}. As $e_{im}$ and $e_{cl}$ usually do not have the same channel number, \ie $C_i\neq C_c$, we use Linear layers to align the dimensions between the descriptors from two image encoders: 
\begin{equation}
    \begin{aligned}
        \mathcal{L}_{far}&(e_{im}, e_{cl}) = \|\mathbb{T}_a\cdot S_{avg}(e_{im}) - S_{avg}(e_{cl})\|_\mathcal{F}\\
    &+ \|\mathbb{T}_m\cdot S_{max}(e_{im}) - S_{max}(e_{cl})\|_\mathcal{F},
    \end{aligned}
    \label{eq:far}
\end{equation}
$\mathbb{T}_a$ and $\mathbb{T}_m$ refer to the learnable Linear layers, and $\|\cdot\|_\mathcal{F}$ is the Frobenius norm.

The pretraining stage minimizes $\Phi_{far}(Y^s_{gt})$ to optimize the self-supervision loss on ground truth images of the synthetic dataset, which are of natural image distribution. During finetuning of $\mathrm{M}$, we also minimize $\Phi_{far}(\mathrm{M}(X^r))$ to constraint the disparity of distribution between $\mathrm{M}(X^r)$ and natural images that have been optimized for. 


==> tables/compare_quant.tex <==
\begin{table*}[h]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{c|c|ccc|ccc|ccc|ccc}
    \hline
    \hline
       \multirow{2}{*}{Datasets} & \multirow{2}{*}{Metrics}&\multicolumn{3}{c|}{CNN-based}&\multicolumn{3}{c|}{Transformer-based}&\multicolumn{3}{c|}{VQ-based}&\multicolumn{3}{c}{Diffusion-based}  \\
        \cline{3-14}
        & & RealESRGAN+& +LWay (B.) &+Ours&SwinIRGAN& +LWay (B.) &+Ours&FeMaSR& +LWay (B.) &+Ours&StableSR& +LWay (B.)&+Ours\\
        \hline
        \multirow{6}{*}{NTIRE20}&PSNR$\uparrow$&25.08 & & & 26.93& & &23.54 & & &23.88 & & \\
        &SSIM$\uparrow$&0.7061 & & &0.7467 & & &0.6665& & &0.6482 & & \\
        &LPIPS$\downarrow$&0.2504 & & &0.2290 & & & 0.2360& & &0.2403 & & \\
        &NLPD$\downarrow$&0.3310 & & &0.783 & & &0.3735 & & &0.3909 & & \\
        &DISTIS$\downarrow$&0.1326 & & &0.1200 & & &0.1297 & & & 0.1793& & \\
        &NRQM$\uparrow$&6.121 & & &5.740 & & & 6.625& & &7.653 & & \\
        \hline
        \hline
        \multirow{6}{*}{\makecell[c]{RealSR-\\Canon}}&PSNR$\uparrow$&24.74 & & &26.77 & & &24.29 & & & 24.22& & \\
        &SSIM$\uparrow$&0.7643 & & &0.7892 & & &0.7460 & & &0.7331 & & \\
        &LPIPS$\downarrow$&0.2607 & & &0.2576 & & &0.2809 & & &0.2732 & & \\
        &NLPD$\downarrow$&0.3490 & & &0.3071 & & &0.3652 & & &0.3810& & \\
        &DISTIS$\downarrow$&0.1609 & & &0.1606 & & &0.1884 & & &0.1970 & & \\
        &NRQM$\uparrow$&6.065 & & & 4.225& & &6.015 & & &7.379 & & \\
        \hline
        \multirow{6}{*}{\makecell[c]{RealSR-\\Nikon}}&PSNR$\uparrow$&24.31 & & &26.25 & & &23.94 & & &23.83 & & \\
        &SSIM$\uparrow$&0.7334 & & &0.7602 & & & 0.7097& & &0.6813& & \\
        &LPIPS$\downarrow$&0.2851 & & &0.2796 & & & 0.3046& & &0.3013& & \\
        &NLPD$\downarrow$&0.3476 & & &0.3074 & & &0.3668 & & &0.3909& & \\
        &DISTIS$\downarrow$&0.1760 & & &0.1707 & & &0.1997 & & &0.2269 & & \\
        &NRQM$\uparrow$&5.669 & & &4.854 & & & 5.949& & &7.234 & & \\
        \hline
        \hline
        \multirow{6}{*}{\makecell[c]{DRealSR-\\Sony}}&PSNR$\uparrow$&26.65 & & &30.41 & & &25.93 & & &27.30 & & \\
        &SSIM$\uparrow$&0.8033 & & &0.8499 & & & 0.7671& & &0.7382 & & \\
        &LPIPS$\downarrow$&0.2707 & & &0.2429 & & &0.3143 & & &0.3290 & & \\
        &NLPD$\downarrow$&0.2949 & & &0.2614 & & &0.3399 & & & 0.3473& & \\
        &DISTIS$\downarrow$&0.1515 & & &0.1501 & & &0.2021 & & &0.2272 & & \\
        &NRQM$\uparrow$&5.292 & & &4.387 & & &5.909 & & &7.216 & & \\
        \hline
        \multirow{6}{*}{\makecell[c]{DRealSR-\\Olympus}}&PSNR$\uparrow$&26.73 & & &28.35 & & &24.38 & & &27.36 & & \\
        &SSIM$\uparrow$&0.7667 & & &0.7965 & & &0.6691 & & & 0.7135& & \\
        &LPIPS$\downarrow$&0.3159& & &0.3566 & & &0.4007 & & &0.3822 & & \\
        &NLPD$\downarrow$&0.3117 & & &0.2830 & & &0.3910 & & &0.3376 & & \\
        &DISTIS$\downarrow$&0.1672 & & &0.1979 & & &0.2126 & & &0.2412 & & \\
        &NRQM$\uparrow$& 5.253& & & & & &6.259 & & &7.036 & & \\
        \hline
        \multirow{6}{*}{\makecell[c]{DRealSR-\\Panasonic}}&PSNR$\uparrow$&27.03 & & &28.58 & & & 25.02& & &27.67 & & \\
        &SSIM$\uparrow$&0.7782 & & &0.7998 & & &0.7118 & & &0.7054 & & \\
        &LPIPS$\downarrow$&0.2703 & & &0.2685 & & &0.3088 & & &0.3143 & & \\
        &NLPD$\downarrow$&0.3129 & & &0.2856 & & &0.3685 & & &0.3473 & & \\
        &DISTIS$\downarrow$&0.1588 & & &0.1697 & & &0.1803 & & &0.2240 & & \\
        &NRQM$\uparrow$&5.375 & & &4.534 & & &6.034 & & &6.948 & & \\
        \hline
        \hline
    \end{tabular}}
    \caption{Caption}
    \label{tab:my_label}
\end{table*}
